Stochastic Variance-Reduced Cubic Regularization for Nonconvex Optimization

Cubic regularization (CR) is an optimization method with emerging popularity due to its capability to escape saddle points and converge to second-order stationary solutions for nonconvex optimization. However, CR encounters a high sample complexity issue for finite-sum problems with a large data size. %Various inexact variants of CR have been proposed to improve the sample complexity. In this paper, we propose a stochastic variance-reduced cubic-regularization (SVRC) method under random sampling, and study its convergence guarantee as well as sample complexity. We show that the iteration complexity of SVRC for achieving a second-order stationary solution within $\epsilon$ accuracy is $O(\epsilon^{-3/2})$, which matches the state-of-art result on CR types of methods. Moreover, our proposed variance reduction scheme significantly reduces the per-iteration sample complexity. The resulting total Hessian sample complexity of our SVRC is ${\Oc}(N^{2/3} \epsilon^{-3/2})$, which outperforms the state-of-art result by a factor of $O(N^{2/15})$. We also study our SVRC under random sampling without replacement scheme, which yields a lower per-iteration sample complexity, and hence justifies its practical applicability.

==> Experiment.tex <==
\vspace{-.1cm}
\section{Experimental Results}\label{sec:experiment}
\vspace{-.1cm}
In this section, we compare the performance of SVRC (in fact, its implementation version SVRC$^+$) with a few other competitive algorithms. 
We solve a logistic regression problem with the nonconvex regularizer $\lambda \sum_{i=1}^{d} x_{i}^2/(1 +x_{i}^2 )$ \cite{Antoniadis_2011} over the a9a dataset \cite{Chang_2011}, where $x_i$ denotes the $i$-th coordinate of $\x$. The data set contains a total number $n = 32561$ of samples with the feature dimension $d = 123$.  
	 
We compare among the following five algorithms: SCR under sampling without replacement (\textbf{SCR\_without}), SCR under sampling with replacement but with truncation of the sample size by the total number of samples as implemented in \cite{kohler2017} (\textbf{SCR\_with\_t}), SCR under uniform sampling \footnote{\cite{Xu2017} also proposed a non-uniform sampling scheme, which we do not implement, because we compare here only among uniform sampling schemes. The non-uniform sampling scheme can be explored for both SCR and SVRC as well as an independent effort.} with replacement with a constant sample size as studied in \cite{Xu2017} (\textbf{SCR\_with\_c}), SVRC$^+$ under sampling without replacement (\textbf{SVRC$^+$\_without}), and SVRC$^+$ under sampling without replacement with a constant sample size (\textbf{SVRC$^+$\_without\_c}). For all experiments, we sub-sample only Hessian for simplicity as it dominates the overall complexity. The results with sampling both Hessian and gradient are similar. Furthermore, to implement SVRC, since the Hessian sample size $|\xi_{H}(k)|$ depends on $\s_{k+1}$ which cannot be determined at the $k$-th iteration, we use $\s_k$ as an estimator as suggested in \cite{kohler2017}. Furthermore, since the Hessian Lipschitz constant is unknown, we use the adaptive procedure and solve the cubic sub-problem in the Krylov subspace, as suggested in \cite{Cartis2011a,kohler2017}.  
     
The experimental results are summarized in \Cref{experiment_result}. In specific, \Cref{experiment_result} (a) compares the time efficiency of the five algorithms. It can be seen that the two SVRC$^+$ algorithms start to converge faster than other SCR algorithms in time from a certain point, which can be explained by the fact that SVRC$^+$ algorithms enter the variance reduced phase from such a point. This demonstrates the practical advantage of the variance reduction scheme particularly when the algorithm is close to convergence. \Cref{experiment_result} (a) also indicates that SVRC$^+$ with a constant sample size performs the best, further demonstrating that the variance reduction scheme is powerful enough performs well in practice so that there is even no need to adapt sample size to approximate Hessian. 

\begin{figure} 
	\centering 
		\subfigure[]{\includegraphics[width=0.45\linewidth]{figure/1_gradient_norm_vs_times.pdf}}  
	\subfigure[]{ \includegraphics[width=0.45\linewidth]{figure/1_grad_norm_vs_computation.pdf}}  
	\subfigure[]{ \includegraphics[width=0.45\linewidth]{figure/1_grad_norm_vs_iteration.pdf}}
	\subfigure[]{ \includegraphics[width=0.45\linewidth]{figure/4_gradient_norm_vs_times.pdf}}  \vspace{-3mm}
	\caption{(a): Comparison of time efficiency. (b): Comparison of sample complexity.
	(c): Comparison of iteration complexity. (d): Comparison between sampling with and without replacement.} \label{experiment_result}	
\vspace{-5mm}	
\end{figure}

\Cref{experiment_result} (b) compares the convergence rate of the five algorithms as a function of the total Hessian sample complexity. One can see that the two SVRC$^+$ algorithms have better sample complexity than SCR\_without and SCR\_with\_t, whereas SCR\_with\_c achieves the best sample complexity. For the two SVRC algorithms, the variance reduction scheme comes into effect at roughly 1.5 passes over the data, after which both algorithms have a very sharp drop down in sample size. This implies that inner loops are quite sample efficient with the variance reduction scheme. For SCR\_with\_c, although it requires the least number of Hessian samples, its iteration complexity is much worse than that of other algorithms, as can be seen from \Cref{experiment_result} (c). This implies that SCR\_with\_c makes a slow progress per-iteration, and consequently has a overall low time efficiency as shown in (a). 

In \Cref{experiment_result} (d), we further compare the time efficiency between two sampling schemes, i.e., with and without replacement. We compare these two sampling schemes for both SCR and SVRC$^+$ algorithms. It can be seen that SCR\_without and SVRC$^+$\_without perform better than their counterparts SCR\_with and SVRC$^+$\_with, respectively. This corroborates our theoretical finding of the advantage of sampling without replacement over sampling with replacement.  



\textbf{Sample Batch Size Choices:} The estimation of batch sample size in \cref{eq:svrc_nrep_g} and others for iteration $k$ depends on the step size $\norml{\x_{k+1} - \x_{k}}$, which has not been determined yet.  Fortunately, as shown in \cite{kohler2017}, the previous stepsize is a good estimator of the current one. Moreover, comparing to this adaptive step size, a more conservative but constant step size may be used. We can use the lower bound $\epsilon$ as the value of $\norml{\x_{k+1} - \x_{k}}$. It is not hard to verify that our theoretical results also hold for this conservative choice. We choose the adaptive step size as our presentation due to the adaptive size may be more efficient in practice.
 



